Asymptotic Log-Det Sum-of-Ranks Minimization via Tensor (Alternating) Iteratively Reweighted Least Squares

Affine sum-of-ranks minimization (ASRM) generalizes the affine rank minimization (ARM) problem from matrices to tensors. Here, the interest lies in the ranks of a family $\mathcal{K}$ of different matricizations. Transferring our priorly discussed results on asymptotic log-det rank minimization, we show that iteratively reweighted least squares with weight strength $p = 0$ remains a, theoretically and practically, particularly viable method denoted as $\mathrm{IRLS}$-$0\mathcal{K}$. As in the matrix case, we prove global convergence of asymptotic minimizers of the log-det sum-of-ranks function to desired solutions. Further, we show local convergence of $\mathrm{IRLS}$-$0\mathcal{K}$ in dependence of the rate of decline of the therein appearing regularization parameter $\gamma \searrow 0$. For hierarchical families $\mathcal{K}$, we show how an alternating version ($\mathrm{AIRLS}$-$0\mathcal{K}$, related to prior work under the name $\mathrm{SALSA}$) can be evaluated solely through tensor tree network based operations. The method can thereby be applied to high dimensions through the avoidance of exponential computational complexity. Further, the otherwise crucial rank adaption process becomes essentially superfluous even for completion problems. In numerical experiments, we show that the therefor required subspace restrictions and relaxation of the affine constraint cause only a marginal loss of approximation quality. On the other hand, we demonstrate that $\mathrm{IRLS}$-$0\mathcal{K}$ allows to observe the theoretical phase transition also for generic tensor recoverability in practice. Concludingly, we apply $\mathrm{AIRLS}$-$0\mathcal{K}$ to larger scale problems.

==> tables/table_10_HT_completion_by_method.tex <==
\definecolor{temporarytablecolor1}{RGB}{246,168,0}
\definecolor{temporarytablecolor2}{RGB}{250,190,80}
\definecolor{temporarytablecolor3}{RGB}{214,188,95}
\definecolor{temporarytablecolor4}{RGB}{236,211,152}
\begin{tabular}{ll||c |rcl|cc}
\multirow{2}{*}{instance} & \multicolumn{1}{r||}{ASRM-$\mathcal{K}_{\mathrm{bbHT}}$:} & $\mathcal{Q}_{\varepsilon} \in [0,0.98]$ & \multicolumn{3}{c|}{$\mathcal{Q}_{\varepsilon} \in (0.98,1.005)$} & $\mathcal{Q}_{\varepsilon} \in [1.005,\infty)$ & $\mathcal{Q}_{\varepsilon} = \infty$ \\
& \multicolumn{1}{r||}{recovery:} & \cross & \cross &  & \cmark & \multicolumn{2}{c}{\cross} \\
\hline
\hline
\multirow{4}{*}{${\ell = 69}$}
& {\color{temporarytablecolor1}$\bullet$} (a) full, image & \rcint{  0}{0} & \rcint{  0}{0} & + & \rcint{  0}{0} & \rcint{  0}{0} & \rcint{100}{0}  \\
& {\color{temporarytablecolor2}$\bullet$} (b) full, relaxed & \rcint{  0}{0} & \rcint{  0}{0} & + & \rcint{  0}{0} & \rcint{  0}{0} & \rcint{100}{0}  \\
& {\color{temporarytablecolor3}$\bullet$} (c) alternating, rank fixed & \rcint{  0}{0} & \rcint{  0}{0} & + & \rcint{  0}{0} & \rcint{  0}{0} & \rcint{100}{0}  \\
& {\color{temporarytablecolor4}$\bullet$} (d) alternating, rank adapted & \rcint{  0}{0} & \rcint{  0}{0} & + & \rcint{  0}{0} & \rcint{  0}{0} & \rcint{100}{0}  \\
\hline
\multirow{4}{*}{${\ell = 83}$}
& {\color{temporarytablecolor1}$\bullet$} (a) full, image & \rcint{  0}{0} & \rcint{  0}{0} & + & \rcint{ 33}{0} & \rcint{  0}{0} & \rcint{ 67}{0}  \\
& {\color{temporarytablecolor2}$\bullet$} (b) full, relaxed & \rcint{  0}{0} & \rcint{  0}{0} & + & \rcint{ 33}{0} & \rcint{  0}{0} & \rcint{ 67}{0}  \\
& {\color{temporarytablecolor3}$\bullet$} (c) alternating, rank fixed & \rcint{  0}{0} & \rcint{  0}{0} & + & \rcint{ 15}{0} & \rcint{  0}{0} & \rcint{ 85}{0}  \\
& {\color{temporarytablecolor4}$\bullet$} (d) alternating, rank adapted & \rcint{  0}{0} & \rcint{  0}{0} & + & \rcint{ 14}{0} & \rcint{  0}{0} & \rcint{ 86}{0}  \\
\hline
\multirow{4}{*}{${\ell = 111}$}
& {\color{temporarytablecolor1}$\bullet$} (a) full, image & \rcint{  0}{0} & \rcint{  0}{0} & + & \rcint{ 94}{0} & \rcint{  0}{0} & \rcint{  6}{0}  \\
& {\color{temporarytablecolor2}$\bullet$} (b) full, relaxed & \rcint{  0}{0} & \rcint{  0}{0} & + & \rcint{ 94}{0} & \rcint{  0}{0} & \rcint{  6}{0}  \\
& {\color{temporarytablecolor3}$\bullet$} (c) alternating, rank fixed & \rcint{  0}{0} & \rcint{  0}{0} & + & \rcint{ 96}{0} & \rcint{  0}{0} & \rcint{  4}{0}  \\
& {\color{temporarytablecolor4}$\bullet$} (d) alternating, rank adapted & \rcint{  0}{0} & \rcint{  0}{0} & + & \rcint{ 95}{0} & \rcint{  0}{0} & \rcint{  5}{0}  \\
\hline
\multirow{4}{*}{${\ell = 138}$}
& {\color{temporarytablecolor1}$\bullet$} (a) full, image & \rcint{  0}{0} & \rcint{  0}{0} & + & \rcint{100}{0} & \rcint{  0}{0} & \rcint{  0}{0}  \\
& {\color{temporarytablecolor2}$\bullet$} (b) full, relaxed & \rcint{  0}{0} & \rcint{  0}{0} & + & \rcint{100}{0} & \rcint{  0}{0} & \rcint{  0}{0}  \\
& {\color{temporarytablecolor3}$\bullet$} (c) alternating, rank fixed & \rcint{  0}{0} & \rcint{  0}{0} & + & \rcint{100}{0} & \rcint{  0}{0} & \rcint{  0}{0}  \\
& {\color{temporarytablecolor4}$\bullet$} (d) alternating, rank adapted & \rcint{  0}{0} & \rcint{  0}{0} & + & \rcint{100}{0} & \rcint{  0}{0} & \rcint{  0}{0}  \\
\end{tabular}


==> tables/table_10_HT_completion_by_method_caption.tex <==
\def\temporarycaptioncommand{(A)IRLS-${0\mathcal{K}_{\mathrm{bbHT}}}$ (sampling, d = 4, ${\overline{n} = 5}$, ${\overline{r}_{\mathrm{rs}} = 3}$)}

==> tables/table_7_tensor_by_setting_new.tex <==
\definecolor{temporarytablecolor1}{RGB}{0,84,159}
\definecolor{temporarytablecolor2}{RGB}{155,92,144}
\definecolor{temporarytablecolor3}{RGB}{246,168,0}
\definecolor{temporarytablecolor4}{RGB}{237,120,91}
\begin{tabular}{ll||c |rcl|cc}
\multirow{2}{*}{instance} & \multicolumn{1}{r||}{ASRM-$\mathcal{K}_{\mathrm{bbHT}/\max}$:} & $\mathcal{Q}_{\varepsilon} \in [0,0.98]$ & \multicolumn{3}{c|}{$\mathcal{Q}_{\varepsilon} \in (0.98,1.005)$} & $\mathcal{Q}_{\varepsilon} \in [1.005,\infty)$ & $\mathcal{Q}_{\varepsilon} = \infty$ \\
& \multicolumn{1}{r||}{recovery:} & \cross & \cross &  & \cmark & \multicolumn{2}{c}{\cross} \\
\hline
\hline
\multirow{4}{*}{${c_{\mathrm{mf}} = 1.2}$}
& {\color{temporarytablecolor1}$\bullet$} gaussian, HT, $\ell = 83$ & \rcint{  0}{0} & \rcint{  0}{0} & + & \rcint{ 96}{0} & \rcint{  0}{0} & \rcint{  4}{0}  \\
& {\color{temporarytablecolor2}$\bullet$} gaussian, CP, $\ell = 62$ & \rcint{  0}{0} & \rcint{  0}{0} & + & \rcint{ 18}{0} & \rcint{  0}{0} & \rcint{ 82}{0}  \\
& {\color{temporarytablecolor3}$\bullet$} sampling, HT, $\ell = 83$ & \rcint{  0}{0} & \rcint{  0}{0} & + & \rcint{ 33}{0} & \rcint{  0}{0} & \rcint{ 67}{0}  \\
& {\color{temporarytablecolor4}$\bullet$} sampling, CP, $\ell = 62$ & \rcint{  0}{0} & \rcint{  0}{0} & + & \rcint{  1}{0} & \rcint{  0}{0} & \rcint{ 99}{0}  \\
\hline
\multirow{4}{*}{${c_{\mathrm{mf}} = 1.6}$}
& {\color{temporarytablecolor1}$\bullet$} gaussian, HT, $\ell = 111$ & \rcint{  0}{0} & \rcint{  0}{0} & + & \rcint{100}{0} & \rcint{  0}{0} & \rcint{  0}{0}  \\
& {\color{temporarytablecolor2}$\bullet$} gaussian, CP, $\ell = 82$ & \rcint{  0}{0} & \rcint{  0}{0} & + & \rcint{ 86}{0} & \rcint{  0}{0} & \rcint{ 14}{0}  \\
& {\color{temporarytablecolor3}$\bullet$} sampling, HT, $\ell = 111$ & \rcint{  0}{0} & \rcint{  0}{0} & + & \rcint{ 94}{0} & \rcint{  0}{0} & \rcint{  6}{0}  \\
& {\color{temporarytablecolor4}$\bullet$} sampling, CP, $\ell = 82$ & \rcint{  0}{0} & \rcint{  0}{0} & + & \rcint{ 44}{0} & \rcint{  0}{0} & \rcint{ 56}{0}  \\
\hline
\multirow{4}{*}{${c_{\mathrm{mf}} = 2.0}$}
& {\color{temporarytablecolor1}$\bullet$} gaussian, HT, $\ell = 138$ & \rcint{  0}{0} & \rcint{  0}{0} & + & \rcint{100}{0} & \rcint{  0}{0} & \rcint{  0}{0}  \\
& {\color{temporarytablecolor2}$\bullet$} gaussian, CP, $\ell = 102$ & \rcint{  0}{0} & \rcint{  0}{0} & + & \rcint{100}{0} & \rcint{  0}{0} & \rcint{  0}{0}  \\
& {\color{temporarytablecolor3}$\bullet$} sampling, HT, $\ell = 138$ & \rcint{  0}{0} & \rcint{  0}{0} & + & \rcint{100}{0} & \rcint{  0}{0} & \rcint{  0}{0}  \\
& {\color{temporarytablecolor4}$\bullet$} sampling, CP, $\ell = 102$ & \rcint{  0}{0} & \rcint{  0}{0} & + & \rcint{ 84}{0} & \rcint{  0}{0} & \rcint{ 16}{0}  \\
\end{tabular}


==> tables/table_7_tensor_by_setting_new_caption.tex <==
\def\temporarycaptioncommand{IRLS-${0\mathcal{K}}$ (full, image method, d = 4, ${\overline{n} = 5}$, ${\overline{r}_{\mathrm{rs}} = 3}$)}

==> tables/table_8_tensor_comparison.tex <==
\definecolor{temporarytablecolor1}{RGB}{0,84,159}
\definecolor{temporarytablecolor2}{RGB}{48,140,183}
\definecolor{temporarytablecolor3}{RGB}{141,191,224}
\definecolor{temporarytablecolor4}{RGB}{158,91,105}
\definecolor{temporarytablecolor5}{RGB}{246,168,0}
\definecolor{temporarytablecolor6}{RGB}{214,188,95}
\definecolor{temporarytablecolor7}{RGB}{236,211,152}
\definecolor{temporarytablecolor8}{RGB}{196,104,85}
\begin{tabular}{ll||c |rcl|cc}
\multirow{2}{*}{instance} & \multicolumn{1}{r||}{ASRM-$\mathcal{K}_{\mathrm{Tucker}}$:} & $\mathcal{Q}_{\varepsilon} \in [0,0.98]$ & \multicolumn{3}{c|}{$\mathcal{Q}_{\varepsilon} \in (0.98,1.005)$} & $\mathcal{Q}_{\varepsilon} \in [1.005,\infty)$ & $\mathcal{Q}_{\varepsilon} = \infty$ \\
& \multicolumn{1}{r||}{recovery:} & \cross & \cross &  & \cmark & \multicolumn{2}{c}{\cross} \\
\hline
\hline
\multirow{8}{*}{${\ell = 126}$}
& {\color{temporarytablecolor1}$\bullet$} gaussian ${(r_L = 1)}$: (a) full & \rcint{  0}{0} & \rcint{  0}{0} & + & \rcint{ 99}{0} & \rcint{  0}{0} & \rcint{  1}{0}  \\
& {\color{temporarytablecolor2}$\bullet$} (c) alt & \rcint{  0}{0} & \rcint{  0}{0} & + & \rcint{ 79}{0} & \rcint{  0}{0} & \rcint{ 21}{0}  \\
& {\color{temporarytablecolor3}$\bullet$} (d) alt adapt & \rcint{  0}{0} & \rcint{  0}{0} & + & \rcint{ 78}{0} & \rcint{  0}{0} & \rcint{ 22}{0}  \\
& {\color{temporarytablecolor4}$\bullet$} (e) plain ALS & \rcint{  0}{0} & \rcint{  0}{0} & + & \rcint{  0}{0} & \rcint{  0}{0} & \rcint{100}{0}  \\
& {\color{temporarytablecolor5}$\bullet$} samp: (a) full & \rcint{  0}{0} & \rcint{  0}{0} & + & \rcint{ 89}{0} & \rcint{  0}{0} & \rcint{ 11}{0}  \\
& {\color{temporarytablecolor6}$\bullet$} (c) alt & \rcint{  0}{0} & \rcint{  0}{0} & + & \rcint{ 16}{0} & \rcint{  0}{0} & \rcint{ 84}{0}  \\
& {\color{temporarytablecolor7}$\bullet$} (d) alt adapt & \rcint{  0}{0} & \rcint{  0}{0} & + & \rcint{ 19}{0} & \rcint{  0}{0} & \rcint{ 81}{0}  \\
& {\color{temporarytablecolor8}$\bullet$} (e) plain ALS & \rcint{  0}{0} & \rcint{  0}{0} & + & \rcint{  0}{0} & \rcint{  0}{0} & \rcint{100}{0}  \\
\hline
\multirow{8}{*}{${\ell = 168}$}
& {\color{temporarytablecolor1}$\bullet$} gaussian ${(r_L = 1)}$: (a) full & \rcint{  0}{0} & \rcint{  0}{0} & + & \rcint{100}{0} & \rcint{  0}{0} & \rcint{  0}{0}  \\
& {\color{temporarytablecolor2}$\bullet$} (c) alt & \rcint{  0}{0} & \rcint{  0}{0} & + & \rcint{100}{0} & \rcint{  0}{0} & \rcint{  0}{0}  \\
& {\color{temporarytablecolor3}$\bullet$} (d) alt adapt & \rcint{  0}{0} & \rcint{  0}{0} & + & \rcint{100}{0} & \rcint{  0}{0} & \rcint{  0}{0}  \\
& {\color{temporarytablecolor4}$\bullet$} (e) plain ALS & \rcint{  0}{0} & \rcint{  0}{0} & + & \rcint{ 28}{0} & \rcint{  0}{0} & \rcint{ 72}{0}  \\
& {\color{temporarytablecolor5}$\bullet$} samp: (a) full & \rcint{  0}{0} & \rcint{  0}{0} & + & \rcint{100}{0} & \rcint{  0}{0} & \rcint{  0}{0}  \\
& {\color{temporarytablecolor6}$\bullet$} (c) alt & \rcint{  0}{0} & \rcint{  0}{0} & + & \rcint{ 77}{0} & \rcint{  0}{0} & \rcint{ 23}{0}  \\
& {\color{temporarytablecolor7}$\bullet$} (d) alt adapt & \rcint{  0}{0} & \rcint{  0}{0} & + & \rcint{ 80}{0} & \rcint{  0}{0} & \rcint{ 20}{0}  \\
& {\color{temporarytablecolor8}$\bullet$} (e) plain ALS & \rcint{  0}{0} & \rcint{  0}{0} & + & \rcint{  4}{0} & \rcint{  0}{0} & \rcint{ 96}{0}  \\
\hline
\multirow{8}{*}{${\ell = 210}$}
& {\color{temporarytablecolor1}$\bullet$} gaussian ${(r_L = 1)}$: (a) full & \rcint{  0}{0} & \rcint{  0}{0} & + & \rcint{100}{0} & \rcint{  0}{0} & \rcint{  0}{0}  \\
& {\color{temporarytablecolor2}$\bullet$} (c) alt & \rcint{  0}{0} & \rcint{  0}{0} & + & \rcint{100}{0} & \rcint{  0}{0} & \rcint{  0}{0}  \\
& {\color{temporarytablecolor3}$\bullet$} (d) alt adapt & \rcint{  0}{0} & \rcint{  0}{0} & + & \rcint{100}{0} & \rcint{  0}{0} & \rcint{  0}{0}  \\
& {\color{temporarytablecolor4}$\bullet$} (e) plain ALS & \rcint{  0}{0} & \rcint{  0}{0} & + & \rcint{ 74}{0} & \rcint{  0}{0} & \rcint{ 26}{0}  \\
& {\color{temporarytablecolor5}$\bullet$} samp: (a) full & \rcint{  0}{0} & \rcint{  0}{0} & + & \rcint{100}{0} & \rcint{  0}{0} & \rcint{  0}{0}  \\
& {\color{temporarytablecolor6}$\bullet$} (c) alt & \rcint{  0}{0} & \rcint{  0}{0} & + & \rcint{100}{0} & \rcint{  0}{0} & \rcint{  0}{0}  \\
& {\color{temporarytablecolor7}$\bullet$} (d) alt adapt & \rcint{  0}{0} & \rcint{  0}{0} & + & \rcint{ 98}{0} & \rcint{  0}{0} & \rcint{  2}{0}  \\
& {\color{temporarytablecolor8}$\bullet$} (e) plain ALS & \rcint{  0}{0} & \rcint{  0}{0} & + & \rcint{ 24}{0} & \rcint{  0}{0} & \rcint{ 76}{0}  \\
\end{tabular}


==> tables/table_8_tensor_comparison_caption.tex <==
\def\temporarycaptioncommand{(A)IRLS-${0\mathcal{K}_{\mathrm{Tucker}}}$ (Tucker, d = 4, ${\overline{n} = 5}$, ${\overline{r}_{\mathrm{rs}} = 3}$)}

==> tables/table_9_alternating_tensor_by_setting.tex <==
\definecolor{temporarytablecolor1}{RGB}{118,163,144}
\definecolor{temporarytablecolor2}{RGB}{182,200,191}
\definecolor{temporarytablecolor3}{RGB}{71,147,170}
\definecolor{temporarytablecolor4}{RGB}{155,194,213}
\begin{tabular}{ll||c |rcl|cc}
\multirow{2}{*}{instance} & \multicolumn{1}{r||}{ASRM-$\mathcal{K}_{\mathrm{bbHT}}$:} & $\mathcal{Q}_{\varepsilon} \in [0,0.98]$ & \multicolumn{3}{c|}{$\mathcal{Q}_{\varepsilon} \in (0.98,1.005)$} & $\mathcal{Q}_{\varepsilon} \in [1.005,\infty)$ & $\mathcal{Q}_{\varepsilon} = \infty$ \\
& \multicolumn{1}{r||}{recovery:} & \cross & \cross &  & \cmark & \multicolumn{2}{c}{\cross} \\
\hline
\hline
\multirow{4}{*}{${\ell = 13000}$}
& {\color{temporarytablecolor1}$\bullet$} gaussian ($r_L = 1$) & \rcint{  0}{0} & \rcint{  0}{0} & + & \rcint{  0}{0} & \rcint{  0}{0} & \rcint{100}{0}  \\
& {\color{temporarytablecolor2}$\bullet$} gaussian ($r_L = 1$), neigh & \rcint{  0}{0} & \rcint{  0}{0} & + & \rcint{  0}{0} & \rcint{  0}{0} & \rcint{100}{0}  \\
& {\color{temporarytablecolor3}$\bullet$} gaussian ($r_L = 2$) & \rcint{  0}{0} & \rcint{  0}{0} & + & \rcint{  0}{0} & \rcint{  0}{0} & \rcint{100}{0}  \\
& {\color{temporarytablecolor4}$\bullet$} gaussian ($r_L = 2$), neigh & \rcint{  0}{0} & \rcint{  0}{0} & + & \rcint{  0}{0} & \rcint{  0}{0} & \rcint{100}{0}  \\
\hline
\multirow{4}{*}{${\ell = 19500}$}
& {\color{temporarytablecolor1}$\bullet$} gaussian ($r_L = 1$) & \rcint{  0}{0} & \rcint{  0}{0} & + & \rcint{ 19}{0} & \rcint{  0}{0} & \rcint{ 81}{0}  \\
& {\color{temporarytablecolor2}$\bullet$} gaussian ($r_L = 1$), neigh & \rcint{  0}{0} & \rcint{  0}{0} & + & \rcint{  1}{0} & \rcint{  0}{0} & \rcint{ 99}{0}  \\
& {\color{temporarytablecolor3}$\bullet$} gaussian ($r_L = 2$) & \rcint{  0}{0} & \rcint{  0}{0} & + & \rcint{ 32}{0} & \rcint{  0}{0} & \rcint{ 68}{0}  \\
& {\color{temporarytablecolor4}$\bullet$} gaussian ($r_L = 2$), neigh & \rcint{  0}{0} & \rcint{  0}{0} & + & \rcint{  6}{0} & \rcint{  0}{0} & \rcint{ 94}{0}  \\
\hline
\multirow{4}{*}{${\ell = 26000}$}
& {\color{temporarytablecolor1}$\bullet$} gaussian ($r_L = 1$) & \rcint{  0}{0} & \rcint{  0}{0} & + & \rcint{ 89}{0} & \rcint{  0}{0} & \rcint{ 11}{0}  \\
& {\color{temporarytablecolor2}$\bullet$} gaussian ($r_L = 1$), neigh & \rcint{  0}{0} & \rcint{  0}{0} & + & \rcint{ 54}{0} & \rcint{  0}{0} & \rcint{ 46}{0}  \\
& {\color{temporarytablecolor3}$\bullet$} gaussian ($r_L = 2$) & \rcint{  0}{0} & \rcint{  0}{0} & + & \rcint{ 88}{0} & \rcint{  0}{0} & \rcint{ 12}{0}  \\
& {\color{temporarytablecolor4}$\bullet$} gaussian ($r_L = 2$), neigh & \rcint{  0}{0} & \rcint{  0}{0} & + & \rcint{ 73}{0} & \rcint{  0}{0} & \rcint{ 27}{0}  \\
\end{tabular}


==> tables/table_9_alternating_tensor_by_setting_caption.tex <==
\def\temporarycaptioncommand{(A)IRLS-${0\mathcal{K}_{\mathrm{bbHT}}}$ (alternating, with heuristics, d = 8, ${\overline{n} = 20}$, ${\overline{r}_{\mathrm{rs}} = 5}$)}

==> tables/table_9b_alternating_tensor_by_setting_expdec.tex <==
\definecolor{temporarytablecolor1}{RGB}{113,148,142}
\definecolor{temporarytablecolor2}{RGB}{177,188,186}
\definecolor{temporarytablecolor3}{RGB}{78,136,161}
\definecolor{temporarytablecolor4}{RGB}{156,183,202}
\definecolor{temporarytablecolor5}{RGB}{189,164,103}
\definecolor{temporarytablecolor6}{RGB}{218,194,155}
\begin{tabular}{ll||c |rcl|cc}
\multirow{2}{*}{instance} & \multicolumn{1}{r||}{ASRM-$\mathcal{K}_{\mathrm{bbHT}}$:} & $\mathcal{Q}_{\varepsilon} \in [0,0.98]$ & \multicolumn{3}{c|}{$\mathcal{Q}_{\varepsilon} \in (0.98,1.005)$} & $\mathcal{Q}_{\varepsilon} \in [1.005,\infty)$ & $\mathcal{Q}_{\varepsilon} = \infty$ \\
& \multicolumn{1}{r||}{recovery:} & \cross & \cross &  & \cmark & \multicolumn{2}{c}{\cross} \\
\hline
\hline
\multirow{6}{*}{${\ell = 6500}$}
& {\color{temporarytablecolor1}$\bullet$} gaussian ($r_L = 1$) & \rcint{  0}{0} & \rcint{  0}{0} & + & \rcint{ 51}{0} & \rcint{  0}{0} & \rcint{ 49}{0}  \\
& {\color{temporarytablecolor2}$\bullet$} gaussian ($r_L = 1$), neigh & \rcint{  0}{0} & \rcint{  0}{0} & + & \rcint{  9}{0} & \rcint{  0}{0} & \rcint{ 91}{0}  \\
& {\color{temporarytablecolor3}$\bullet$} gaussian ($r_L = 2$) & \rcint{  0}{0} & \rcint{  0}{0} & + & \rcint{ 64}{0} & \rcint{  0}{0} & \rcint{ 36}{0}  \\
& {\color{temporarytablecolor4}$\bullet$} gaussian ($r_L = 2$), neigh & \rcint{  0}{0} & \rcint{  0}{0} & + & \rcint{  5}{0} & \rcint{  0}{0} & \rcint{ 95}{0}  \\
& {\color{temporarytablecolor5}$\bullet$} sampling & \rcint{  0}{0} & \rcint{  0}{0} & + & \rcint{  0}{0} & \rcint{  0}{0} & \rcint{100}{0}  \\
& {\color{temporarytablecolor6}$\bullet$} sampling, neigh & \rcint{  0}{0} & \rcint{  0}{0} & + & \rcint{  0}{0} & \rcint{  0}{0} & \rcint{100}{0}  \\
\hline
\multirow{6}{*}{${\ell = 13000}$}
& {\color{temporarytablecolor1}$\bullet$} gaussian ($r_L = 1$) & \rcint{  0}{0} & \rcint{  0}{0} & + & \rcint{100}{0} & \rcint{  0}{0} & \rcint{  0}{0}  \\
& {\color{temporarytablecolor2}$\bullet$} gaussian ($r_L = 1$), neigh & \rcint{  0}{0} & \rcint{  0}{0} & + & \rcint{ 92}{0} & \rcint{  0}{0} & \rcint{  8}{0}  \\
& {\color{temporarytablecolor3}$\bullet$} gaussian ($r_L = 2$) & \rcint{  0}{0} & \rcint{  0}{0} & + & \rcint{100}{0} & \rcint{  0}{0} & \rcint{  0}{0}  \\
& {\color{temporarytablecolor4}$\bullet$} gaussian ($r_L = 2$), neigh & \rcint{  0}{0} & \rcint{  0}{0} & + & \rcint{ 93}{0} & \rcint{  0}{0} & \rcint{  7}{0}  \\
& {\color{temporarytablecolor5}$\bullet$} sampling & \rcint{  0}{0} & \rcint{  0}{0} & + & \rcint{  0}{0} & \rcint{  0}{0} & \rcint{100}{0}  \\
& {\color{temporarytablecolor6}$\bullet$} sampling, neigh & \rcint{  0}{0} & \rcint{  0}{0} & + & \rcint{  0}{0} & \rcint{  0}{0} & \rcint{100}{0}  \\
\hline
\multirow{6}{*}{${\ell = 19500}$}
& {\color{temporarytablecolor1}$\bullet$} gaussian ($r_L = 1$) & \rcint{  0}{0} & \rcint{  0}{0} & + & \rcint{100}{0} & \rcint{  0}{0} & \rcint{  0}{0}  \\
& {\color{temporarytablecolor2}$\bullet$} gaussian ($r_L = 1$), neigh & \rcint{  0}{0} & \rcint{  0}{0} & + & \rcint{100}{0} & \rcint{  0}{0} & \rcint{  0}{0}  \\
& {\color{temporarytablecolor3}$\bullet$} gaussian ($r_L = 2$) & \rcint{  0}{0} & \rcint{  0}{0} & + & \rcint{100}{0} & \rcint{  0}{0} & \rcint{  0}{0}  \\
& {\color{temporarytablecolor4}$\bullet$} gaussian ($r_L = 2$), neigh & \rcint{  0}{0} & \rcint{  0}{0} & + & \rcint{100}{0} & \rcint{  0}{0} & \rcint{  0}{0}  \\
& {\color{temporarytablecolor5}$\bullet$} sampling & \rcint{  0}{0} & \rcint{  0}{0} & + & \rcint{  0}{0} & \rcint{  0}{0} & \rcint{100}{0}  \\
& {\color{temporarytablecolor6}$\bullet$} sampling, neigh & \rcint{  0}{0} & \rcint{  0}{0} & + & \rcint{  0}{0} & \rcint{  0}{0} & \rcint{100}{0}  \\
\hline
\multirow{6}{*}{${\ell = 26000}$}
& {\color{temporarytablecolor1}$\bullet$} gaussian ($r_L = 1$) & \rcint{  0}{0} & \rcint{  0}{0} & + & \rcint{100}{0} & \rcint{  0}{0} & \rcint{  0}{0}  \\
& {\color{temporarytablecolor2}$\bullet$} gaussian ($r_L = 1$), neigh & \rcint{  0}{0} & \rcint{  0}{0} & + & \rcint{100}{0} & \rcint{  0}{0} & \rcint{  0}{0}  \\
& {\color{temporarytablecolor3}$\bullet$} gaussian ($r_L = 2$) & \rcint{  0}{0} & \rcint{  0}{0} & + & \rcint{100}{0} & \rcint{  0}{0} & \rcint{  0}{0}  \\
& {\color{temporarytablecolor4}$\bullet$} gaussian ($r_L = 2$), neigh & \rcint{  0}{0} & \rcint{  0}{0} & + & \rcint{100}{0} & \rcint{  0}{0} & \rcint{  0}{0}  \\
& {\color{temporarytablecolor5}$\bullet$} sampling & \rcint{  0}{0} & \rcint{  0}{0} & + & \rcint{  0}{0} & \rcint{  0}{0} & \rcint{100}{0}  \\
& {\color{temporarytablecolor6}$\bullet$} sampling, neigh & \rcint{  0}{0} & \rcint{  0}{0} & + & \rcint{  0}{0} & \rcint{  0}{0} & \rcint{100}{0}  \\
\end{tabular}


==> tables/table_9b_alternating_tensor_by_setting_expdec_caption.tex <==
\def\temporarycaptioncommand{(A)IRLS-${0\mathcal{K}_{\mathrm{bbHT}}}$ (alternating, with heuristics, exp. dec. (s = 1/3), d = 8, ${\overline{n} = 20}$, ${\overline{r}_{\mathrm{rs}} = 5}$)}

==> tables/table_n2_tensor_conj_new.tex <==
\definecolor{temporarytablecolor1}{RGB}{0,84,159}
\begin{tabular}{ll||c |rcl|cc}
\multirow{2}{*}{instance} & \multicolumn{1}{r||}{ASRM-$\mathcal{K}$:} & $\mathcal{Q}_{\varepsilon} \in [0,0.98]$ & \multicolumn{3}{c|}{$\mathcal{Q}_{\varepsilon} \in (0.98,1.005)$} & $\mathcal{Q}_{\varepsilon} \in [1.005,\infty)$ & $\mathcal{Q}_{\varepsilon} = \infty$ \\
& \multicolumn{1}{r||}{recovery:} & \cross & \cross &  & \cmark & \multicolumn{2}{c}{\cross} \\
\hline
\hline
\multirow{1}{*}{${\Delta\ell = -1}$}
& {\color{temporarytablecolor1}$\bullet$} HT, $\ell = 68$ & \rcint{ 24}{0} & \rcint{  2}{0} & + & \rcint{  0}{0} & \rcint{ 25}{0} & \rcint{ 49}{0}  \\
\hline
\multirow{1}{*}{${\Delta\ell = 0}$}
& {\color{temporarytablecolor1}$\bullet$} HT, $\ell = 69$ & \rcint{  9}{0} & \rcint{  1}{0} & + & \rcint{  2}{0} & \rcint{  7}{0} & \rcint{ 81}{0}  \\
\hline
\multirow{1}{*}{${\Delta\ell = 1}$}
& {\color{temporarytablecolor1}$\bullet$} HT, $\ell = 70$ & \rcint{  1}{0} & \rcint{  0}{0} & + & \rcint{ 10}{0} & \rcint{  2}{0} & \rcint{ 87}{0}  \\
\end{tabular}


==> tables/table_n2_tensor_conj_new_caption.tex <==
\def\temporarycaptioncommand{tensor recovery (full, Gaussian, image method, d = 4, ${\overline{n} = 5}$, ${\overline{r}_{\mathrm{rs}} = 3}$)}

==> tikz_base_files/Tucker_graph/Tucker_graph.tex <==

\begin{tikzpicture}[network]

  \pgfdeclarelayer{bg}    % declare background layer
  \pgfsetlayers{bg,main}  % set the order of the layers (main is the standard layer)

  \node[tensornode] (C) at (0,0) {$N_{d+1}$};
  \node[tensornode] (U1) at ($(C) + (-150:2)$) {$N_1$};
  \node[tensornode] (U2) at ($(C) + (-110:2)$) {$N_2$};
  \node[tensornode] (U3) at ($(C) + (-70:2)$) {$N_3$};
  \node[tensornode] (U4) at ($(C) + (-30:2)$) {$N_4$};
  
   \node[virtnode] (a1) at ($ (U1) + (-90:\virtnodedist) $) {};
   \node[virtnode] (a2) at ($ (U2) + (-90:\virtnodedist) $) {};
   \node[virtnode] (a3) at ($ (U3) + (-90:\virtnodedist) $) {};
   \node[virtnode] (a4) at ($ (U4) + (-90:\virtnodedist) $) {};
   
  \path[alphacontr,dashed] (U1) edge node[modename] {\color{black}$\alpha_1$} (a1);
  \path[alphacontr,dashed] (U2) edge node[modename] {\color{black}$\alpha_2$} (a2);
  \path[alphacontr,dashed] (U3) edge node[modename] {\color{black}$\alpha_3$} (a3);
  \path[alphacontr,dashed] (U4) edge node[modename] {\color{black}$\alpha_4$} (a4);
  
  \path (C) edge node[modename] {$\scriptscriptstyle \beta^{\{1,d+1\}}$} (U1);
  \path (C) edge node[modename] {$\scriptscriptstyle \beta^{\{2,d+1\}}$} (U2);
  \path (C) edge node[modename] {$\scriptscriptstyle \beta^{\{3,d+1\}}$} (U3);
  \path (C) edge node[modename] {$\scriptscriptstyle \beta^{\{4,d+1\}}$} (U4);
  
  \begin{pgfonlayer}{bg}    % select the background layer
    
    \draw[dotted] \convexpath{U2,C,U4,U3}{0.65cm};
    
  \end{pgfonlayer}
  
  \begin{scope}[shift={(6,0)}]
   
     \pgfdeclarelayer{bg}    % declare background layer
  \pgfsetlayers{bg,main}  % set the order of the layers (main is the standard layer)

  \node[tensornode] (C) at (0,0) {$\widetilde{N}_{d+1}$};
  \node[tensornode] (C2) at (2.5,0) {$\widetilde{N}_{d+2}$};
  \node[tensornode] (U1) at ($(C) + (-150:2)$) {$N_1$};
  \node[tensornode] (U2) at ($(C) + (-110:2)$) {$N_2$};
  \node[tensornode] (U3) at ($(C2) + (-70:2)$) {$N_3$};
  \node[tensornode] (U4) at ($(C2) + (-30:2)$) {$N_4$};
  
   \node[virtnode] (a1) at ($ (U1) + (-90:\virtnodedist) $) {};
   \node[virtnode] (a2) at ($ (U2) + (-90:\virtnodedist) $) {};
   \node[virtnode] (a3) at ($ (U3) + (-90:\virtnodedist) $) {};
   \node[virtnode] (a4) at ($ (U4) + (-90:\virtnodedist) $) {};
   
  \path[alphacontr,dashed] (U1) edge node[modename] {\color{black}$\alpha_1$} (a1);
  \path[alphacontr,dashed] (U2) edge node[modename] {\color{black}$\alpha_2$} (a2);
  \path[alphacontr,dashed] (U3) edge node[modename] {\color{black}$\alpha_3$} (a3);
  \path[alphacontr,dashed] (U4) edge node[modename] {\color{black}$\alpha_4$} (a4);
  
  \path (C) edge node[modename] {$\scriptscriptstyle \beta^{\{1,d+1\}}$} (U1);
  \path (C) edge node[modename] {$\scriptscriptstyle \beta^{\{2,d+1\}}$} (U2);
  \path (C) edge node[modename] {$\scriptscriptstyle \beta^{\{d+1,d+2\}}$} (C2);
  \path (C2) edge node[modename] {$\scriptscriptstyle \beta^{\{3,d+2\}}$} (U3);
  \path (C2) edge node[modename] {$\scriptscriptstyle \beta^{\{4,d+2\}}$} (U4);
  
  \begin{pgfonlayer}{bg}    % select the background layer
    
    \draw[dotted] \convexpath{U1,C,U2}{0.65cm};
    
  \end{pgfonlayer}
   
  \end{scope}

  
\end{tikzpicture}


==> tikz_base_files/Tucker_graphL/Tucker_graphL.tex <==

\begin{tikzpicture}[network]

  \pgfdeclarelayer{bg}    % declare background layer
  \pgfdeclarelayer{ell}
  \pgfsetlayers{ell,bg,main}  % set the order of the layers (main is the standard layer)

  \node[tensornode] (C) at (0,0) {$L_{d+1}$};
  \node[tensornode] (U1) at ($(C) + (-150:2)$) {$L_1$};
  \node[tensornode] (U2) at ($(C) + (-110:2)$) {$L_2$};
  \node[tensornode] (U3) at ($(C) + (-70:2)$) {$L_3$};
  \node[tensornode] (U4) at ($(C) + (-30:2)$) {$L_4$};
  
   \node[virtnode] (a1) at ($ (U1) + (-90:\virtnodedist) $) {};
   \node[virtnode] (a2) at ($ (U2) + (-90:\virtnodedist) $) {};
   \node[virtnode] (a3) at ($ (U3) + (-90:\virtnodedist) $) {};
   \node[virtnode] (a4) at ($ (U4) + (-90:\virtnodedist) $) {};
   
  \path[alphacontr,dashed] (U1) edge node[modename] {\color{black}$\alpha_1$} (a1);
  \path[alphacontr,dashed] (U2) edge node[modename] {\color{black}$\alpha_2$} (a2);
  \path[alphacontr,dashed] (U3) edge node[modename] {\color{black}$\alpha_3$} (a3);
  \path[alphacontr,dashed] (U4) edge node[modename] {\color{black}$\alpha_4$} (a4);
  
  \contourlength{1.5pt}
  
  \path (C) edge node[modename] {\contour{white}{$\scriptscriptstyle \varepsilon^{\{1,d+1\}}$}} (U1);
  \path (C) edge node[modename] {\contour{white}{$\scriptscriptstyle \varepsilon^{\{2,d+1\}}$}} (U2);
  \path (C) edge node[modename] {\contour{white}{$\scriptscriptstyle \varepsilon^{\{3,d+1\}}$}} (U3);
  \path (C) edge node[modename] {\contour{white}{$\scriptscriptstyle \varepsilon^{\{4,d+1\}}$}} (U4);
  
    \begin{pgfonlayer}{bg} 
  \path[line width = 2.5,white] (C) edge (U1);
  \path[line width = 2.5,white] (C) edge (U2);
  \path[line width = 2.5,white] (C) edge (U3);
  \path[line width = 2.5,white] (C) edge (U4);
  
  \node[tensornodeshadow,minimum width = 1.18cm, minimum height = 1.18cm,white] (C) at (0,0) {};
  \node[tensornodeshadow,white] (U1) at ($(C) + (-150:2)$) {};
  \node[tensornodeshadow,white] (U2) at ($(C) + (-110:2)$) {};
  \node[tensornodeshadow,white] (U3) at ($(C) + (-70:2)$) {};
  \node[tensornodeshadow,white] (U4) at ($(C) + (-30:2)$) {};
  \end{pgfonlayer}
  
  \begin{pgfonlayer}{ell} 
  \node[minimum size=0cm] (x) at ($(U1) + (-0.25,1.25)$) {};
  
  \draw[alphacontr,dashed] (U1) to (x.center);
  \draw[alphacontr,dashed] (U2) to (x.center);
  \draw[alphacontr,dashed] (U3) to (x.center);
  \draw[alphacontr,dashed] (U4) to (x.center);
  \end{pgfonlayer}
  
  \node (ell) at ($(x) + (180:\virtnodedist)$) {};
  \path[alphacontr,dashed] (x.center) edge node[modename] {\color{black}$\zeta$} (ell);
  
\end{tikzpicture}

